Fluids with quenched disorder: Scaling of the free energy barrier near critical points

In the context of Monte Carlo simulations, the analysis of the probability distribution $P_L(m)$ of the order parameter $m$, as obtained in simulation boxes of finite linear extension $L$, allows for an easy estimation of the location of the critical point and the critical exponents. For Ising-like systems without quenched disorder, $P_L(m)$ becomes scale invariant at the critical point, where it assumes a characteristic bimodal shape featuring two overlapping peaks. In particular, the ratio between the value of $P_L(m)$ at the peaks ($P_{L, max}$) and the value at the minimum in-between ($P_{L, min}$) becomes $L$-independent at criticality. However, for Ising-like systems with quenched random fields, we argue that instead $\Delta F_L := \ln (P_{L, max} / P_{L, min}) \propto L^\theta$ should be observed, where $\theta>0$ is the "violation of hyperscaling" exponent. Since $\theta$ is substantially non-zero, the scaling of $\Delta F_L$ with system size should be easily detectable in simulations. For two fluid models with quenched disorder, $\Delta F_L$ versus $L$ was measured, and the expected scaling was confirmed. This provides further evidence that fluids with quenched disorder belong to the universality class of the random-field Ising model.

==> Makefile <==
DOCUMENT  = proc
LATEX = pdflatex

fast:
	make pdffigs
	$(LATEX) $(DOCUMENT)

bib:
	make sed
	make veryclean
	$(LATEX) $(DOCUMENT)
	bibtex $(DOCUMENT)
	$(LATEX) $(DOCUMENT)
	$(LATEX) $(DOCUMENT)
	$(LATEX) $(DOCUMENT)

view:
	evince $(DOCUMENT).pdf &

cul:
	make veryclean
	wget -O /dev/null --keep-session-cookies --save-cookies cookies.txt \
        --post-data="username=$(CITEULIKE)&password=$(PASSWORD)&perm=1" http://www.citeulike.org/login.do
	wget -O refs.bib --load-cookies cookies.txt http://www.citeulike.org/bibtex/user/$(CITEULIKE) 
	make bib

sed:
	sed -n -f JOURNAL_AB.sed < refs.bib > refs.bib.tmp
	mv refs.bib.tmp refs.bib

bibstyle:
	tex sfb.dbj

spell:
	aspell --mode=tex -c $(DOCUMENT).tex

pdffigs: $(patsubst %.eps,%.pdf,$(wildcard *.eps))

%.pdf : %.eps
	epstopdf $<

clean:
	rm -f *.aux *.log *.blg *.toc *.out *.fgx *.tbx *.lof *.lot \
              *.dvi *.idx *.ilg *.ind $(DOCUMENT).ps *.end 

veryclean:
	make clean
	rm -f *.bbl

